COARSE: Collaborative Pseudo-Labeling with Coarse Real Labels for Off-Road Semantic Segmentation

Autonomous off-road navigation faces challenges due to diverse, unstructured environments, requiring robust perception with both geometric and semantic understanding. However, scarce densely labeled semantic data limits generalization across domains. Simulated data helps, but introduces domain adaptation issues. We propose COARSE, a semi-supervised domain adaptation framework for off-road semantic segmentation, leveraging sparse, coarse in-domain labels and densely labeled out-of-domain data. Using pretrained vision transformers, we bridge domain gaps with complementary pixel-level and patch-level decoders, enhanced by a collaborative pseudo-labeling strategy on unlabeled data. Evaluations on RUGD and Rellis-3D datasets show significant improvements of 9.7\% and 8.4\% respectively, versus only using coarse data. Tests on real-world off-road vehicle data in a multi-biome setting further demonstrate COARSE's applicability.

==> related_work.tex <==
\section{Related Work}


% \subsection{Pretrained Vision Encoders}

% Pretrained vision encoders have significantly advanced computer vision by enabling robust, transferable feature representations. ResNet \cite{He2015DeepRL} introduced residual connections, addressing the vanishing gradient problem and becoming a standard backbone for deep networks. EfficientNet \cite{Tan2019EfficientNetRM} optimized network scaling to achieve high accuracy with fewer parameters, making it ideal for resource-constrained tasks. MAE \cite{He2021MaskedAA} pioneered Masked Image Modeling (MIM) by reconstructing masked portions of images, leading to effective feature learning without labeled data. DINO \cite{Caron2021EmergingPI} furthered self-supervised learning with a teacher-student framework and the introduction of a multi-crop contrastive learning strategy. Building on DINO, DINOv2 \cite{Oquab2023DINOv2LR} introduced many technical improvements, establishing itself as a state-of-the-art model in self-supervised learning. DINOv2 offers superior performance and adaptability across a large range of tasks.

% \subsection{Semantic Segmentation Architectures}
% Semantic segmentation has been advanced by numerous CNN-based architectures, including FCN \cite{Shelhamer2014FullyCN}, which introduced end-to-end learning for pixel-wise predictions, and U-Net \cite{Ronneberger2015UNetCN}, an encoder-decoder architecture which demonstrated the importance of skip connections. As the field progressed, Vision Transformers have been increasingly adopted, leading to the development of models attention-based models like SETR \cite{Zheng2020RethinkingSS} and Segmenter \cite{Strudel2021SegmenterTF}, which employ self-attention mechanisms for capturing long-range dependencies.  Other models include SegFormer \cite{Xie2021SegFormerSA}, which balances accuracy and efficiency by combining Transformers with lightweight MLP decoders. DPT \cite{Ranftl2021VisionTF} enhances segmentation tasks by incorporating dense skip-connections into Transformers, similar to U-Net, while Mask2Former \cite{Cheng2021MaskedattentionMT} unifies various segmentation tasks under a single framework, leveraging the strengths of both CNNs and Transformers to set new benchmarks in segmentation performance.


% % Swin \cite{Liu2021SwinTH} introduces efficiency improvements with hierarchical feature extraction with shifted windows.

% \subsection{Data-Scarce Semantic Segmentation}
% One of the main challenges of deep learning approaches for semantic segmentation is the limited amount of labeled real data. Many different approaches exist depending on the availability of certain data types. In the Semi-Supervised setting, ClassMix \cite{Olsson2020ClassMixSD} uses unlabeled samples by mixing semantic masks from predictions to produce pseudo-labels. \cite{Hoyer2020ThreeWT} utilize self-supervised depth estimation and improve on ClassMix with DepthMix by mixing semantic masks based on geometric consistency in the scene. Cross Teaching \cite{Luo2021SemiSupervisedMI} implement an end-to-
% end supervision strategy by using the predictions from a CNN and a Transformer as a supervision signal for each other.

% Unfortunately, dense semantic labels may often be expensive in time (up to 90 minutes per image) as compared to their coarse counterparts (around 7 minutes per image) \cite{Das2022UrbanSS}. \cite{Luo2018CoarsetoFineAE} use a clustering approach to expand the semantics, while \cite{Das2022UrbanSS} first train a model on available coarse and simulation data, and densify coarse labels in highly confident areas of test-time augmentations.

% Another research direction attempts to exploit the generous availability of simulation data to improve models in a data-scarce environment. Similar to ClassMix, DACS \cite{Tranheden2020DACSDA} creates augmented samples by mixing semantic masks and corresponding images between simulation and real domain. CORDA \cite{Wang2021DomainAS} builds upon it by using the correlation between depth and semantic information to help facilitate  domain transfer. DAFormer \cite{Hoyer2021DAFormerIN} utilizes the SegFormer \cite{Xie2021SegFormerSA} architecture and the mean-teacher paradigm to significantly improve the adaptation. Finally, HRDA \cite{Hoyer2022HRDACH} and \cite{Hoyer2022MICMI} go a few step further by including multi-resolution training, respectively Masked Image Modeling to enhance details as well as context consistencies.

% \subsection{Off-Road Semantic Segmentation}

% % talk about classical semantic segmentaton
% % talk about self-supervised methods
% As opposed to the urban application, the off-road semantic segmentation challenge presents large environment differences between different domains. Existing methods mainly solve challenge for each domain individually. Notably, \cite{Sharma2019SemanticSW} pretrain a CNN on simulation data before finetuning on real data. GA-Nav \cite{Guan2021GANavGA} utilize the SegFormer encoder and a custom decoding architecture to obtain state-of-the-art results in both accuracy and performance on a specific class-combination of RUGD and RELLIS-3D. OFFSEG \cite{Viswanath2021OFFSEGAS} utilize a two-step approach to tackle the off-road segmentation challenge. The world is first segmented into 4 high level classes informing on the traversability, and the information is further processed into sub-classes more fine-grained scene understanding.
% In addition to mainly tackling each domain separately, these methods also display one big issue among segmentation datasets: the variability in class definitions across environments. Indeed, off-road segmentation datasets do not share all classes, and the developed methods are usually tested on a specific subset of classes, rendering comparisons potentially difficult.

% or prone to errors around semantic boundaries, especially in the off-road case. Coarse labels on the other hand are much easier produce. 

% % \textcolor{red}{include racer semantic paper once it gets published somewhere} We build upon this work and extend it by 
% % \begin{enumerate}
% %     \item Present a method for selecting new images to label judiciously with DINOv2
% %     \item Utilize large amounts of unlabeled data in addition to few-shot labels in new environments
% %     \item split the semantic mapping problem into environment + obstacle detection problem, designing models specifically to tackle each one.
% % \end{enumerate}

